When Are Learned Models Better Than Hash Functions?

In this work, we aim to study when learned models are better hash functions, particular for hash-maps. We use lightweight piece-wise linear models to replace the hash functions as they have small inference times and are sufficiently general to capture complex distributions. We analyze the learned models in terms of: the model inference time and the number of collisions. Surprisingly, we found that learned models are not much slower to compute than hash functions if optimized correctly. However, it turns out that learned models can only reduce the number of collisions (i.e., the number of times different keys have the same hash value) if the model is able to over-fit to the data; otherwise, it can not be better than an ordinary hash function. Hence, how much better a learned model is in avoiding collisions highly depends on the data and the ability of the model to over-fit. To evaluate the effectiveness of learned models, we used them as hash functions in the bucket chaining and Cuckoo hash tables. For bucket chaining hash table, we found that learned models can achieve 30% smaller sizes and 10% lower probe latency. For Cuckoo hash tables, in some datasets, learned models can increase the ratio of keys stored in their primary locations by around 10%. In summary, we found that learned models can indeed outperform hash functions but only for certain data distributions and with a limited margin.

==> Learned Hashing/analysis.tex <==
\vspace{-5pt}
\section{Analysis of Learned Models}

\input{analysis_models_for_less_collisions}
\input{analysis_models_as_fast_hash_functions}

==> Learned Hashing/analysis_models_as_fast_hash_functions.tex <==
\subsection{Can Learned Models be Computationally as Fast as Traditional Hash Functions?}

In this section, we first present the computation bottleneck of using learned models as hash functions. Then, we discuss the opportunity of alleviating such bottleneck by using vectorization (i.e., Single Instruction Multiple Data ({\simd}) instructions) and prefetching-optimized inter-task parallelism techniques (e.g., {\amac}~\cite{KFG15}). 

\noindent\textbf{Cache Misses Overhead.} The computation of traditional hash functions is fast. It usually includes the execution of arithmetic, logical, and shifting operations (e.g., Multiply-shift~\cite{DHK+97}, and Murmur~\cite{RAD15}). %, Multiply-add-shift~\cite{Die18} ... This makes them a natural fit for direct {\simd} implementations as well as automatic vectorization in recent compilers (e.g., GCC and ICC), and hence their throughput can be increased significantly. 
In contrast, using learned models, like {\rmi}, as a hash function incurs higher latency. The main reason is that, although the inference computation of these models (which is basically the hashing computation in our case) is completely based on arithmetic operations (e.g., add, multiply, max), there is an additional overhead in accessing the model parameters (e.g., intercepts and slopes) that will be used during the computation. This overhead significantly increases if the model size becomes large as its parameters will not completely fit in the cache, and randomly accessing them from the memory will incur many cache misses.  

\noindent\textbf{Performance Gain via {\simd}.}
Interestingly, vectorizing the computation in learned models is \textit{more efficient} than vectorizing some hash functions \textit{as long as the model parameters are kept warm in the cache}. To backup this claim, we micro-benchmarked the throughput of hashing 128 million 64-bit integer keys using a single-threaded {\avx} {\simd} implementation for both Murmur~\cite{Murmur3} and 2-levels {\rmi} model~\cite{KBC+18}, running on a machine with Intel(R) Xeon(R) processors (Skylake architecture). %We chose Murmur to compare against as it is well-known for its good balance between computation time and collision rates in addition to being widely-used in database systems~\cite{RAD15} \footnote{Multiply-shift is faster than Murmur, yet, has higher collision rates in many cases.}. 
We made sure that all models' parameters are kept in the cache by building an {\rmi} with a total of 5 linear models only (1 root model, and 4 models in the second level). Our results showed that the hashing throughputs for vectorized {\rmi} and vectorized Murmur are 1000 and 800 million keys/sec, respectively. This is expected because, \textit{with ignoring the effect of parameters' cache misses}, the inference computation (i.e., hashing) in {\rmi} heavily relies on fast comparison (e.g., min/max) and fused instructions\footnote{Intel(R) Xeon(R) Gold 6230 processor has two physical {\avx} FMA units.} (e.g., fmadd), each has a throughput of 2 instructions/cycle~\cite{IntelIntrinsics}. On the other hand, 60\% of the total instructions needed in the Murmur computation have a throughput of 1 instruction/cycle or less, such as logical shift (1 instruction/cycle) and multiplication (0.66 instruction/cycle). 

\noindent\textbf{Performance Gain via {\amac}.}
As previously mentioned, the superiority of vectorized learned models quickly diminishes when we have large models, which is a typical case in real settings. In this case, the model parameters are frequently accessed from memory and not from cache. Even if some of the requested parameters from a vectorized instruction hit in cache, the instruction cannot proceed until cache misses of the other parameters in the vector are resolved. Obviously, direct software prefetching is not a feasible solution to this issue, and will completely stall the performance, because the model parameters require immediate memory access. Therefore, we propose to hide the cache misses latency by combining the vectorized learned models with a widely-used prefetching-optimized inter-task parallelism technique, namely {\amac}~\cite{KFG15}. This helps in making the overall latency of vectorized learned models very close to traditional hash functions as shown in our evaluation (Section~\ref{sec:evaluation}).
%Basically, {\amac} builds a Finite State Machine ({\fsm}) for each task, where each state in the task, except the last state, ends by a memory prefetching. {\amac} runs different instances of the {\fsm} independently, yet interleavingly, and each running instance transitions among its internal states circularly. Since the overhead of maintaining the {\fsm}s in {\amac} is light compared to the overhead of cache misses~\cite{KFG15}, the overall latency of vectorized learned models and traditional hash functions will still be very close as shown in our evaluation (Section~\ref{sec:evaluation}).
Appendix~\ref{app:hash_via_learned_models_algo} shows our proposed batch-oriented hash function that combines the benefits of {\simd} and {\amac} with learned models.


==> Learned Hashing/analysis_models_for_less_collisions.tex <==
%\subsection{Can Learned Models led to lesser collisions?}
\subsection{Can Learned Models Cause Less Collisions?}
\label{sec:analysis_collisions}
    %\kapil{mention good hash function}
    %\kapil{define notation first}


In this section, we first characterize collisions and then use this to identify/analyze factors affecting collisions for learned models and hash functions.
This analysis helps us to characterize situations where learned models outperform hash functions.

\noindent\textbf{Notation.} We consider the task of mapping $N$ keys to $N$ locations for ease of analysis.
$x_0,x_1,...$ is the sorted array of $N$ keys ($x_i<=x_{i+1}$) and $y_0,y_1,..$, where $y_i\in[0,N-1]$, is the corresponding sorted array of output values ( $y_j=f(x_i)$) where f is a learned model or hash function) such that $y_i<=y_{i+1}$. 
%\ak{I don't understand what we mean by output values. I think it would help to add a little example here. Also, why sort them separately from the keys? I really don't get it. Aren't these just the locations? Why call them output values? I think I confused it with values in a hash table?}
Note that $x_i$ does not necessarily relate to $y_i$, $x_i$'s and $y_i$'s are just sorted versions of the original input keys and output locations.
For learned models, $y_i$'s are continuous values and the precise output location is the closest integer to $y_i$'s.
The sorted output values generate a set of gaps $g_1, g_2,...$ such that $y_i=\left(\sum_{t=1}^i g_t\right)+y_0$.
These gaps form a distribution $G$ with a probability density function (PDF) $f_{G}$.
The discussion and analysis in the rest of this section support the following points:
%The main points we make in this section are:
\begin{itemize}
    \item Collisions are dependent on the gaps between consecutive sorted output values ($g_i$'s).
   
    \item For piece-wise linear models, the number of collisions is dependent on the key distribution, specifically the gaps between consecutive sorted keys ($x_{i}-x_{i-1}$). Higher variation in the distribution of gaps between keys leads to more collisions. Having more linear models improves the accuracy but may not reduce the collisions.
    \item Collisions for a good hash function are independent of the input key distribution (The distribution of $x_i$'s).
\end{itemize}

%These points are discussed in order in the following subsections.

\noindent\textbf{Characterizing Collisions.}
If two keys are mapped to the same location, then there is a collision.
The key insight regarding collisions is that the collisions depend on the gaps between consecutive output values (${y_i-y_{i-1}}$).
If the gap between two consecutive output values is greater than one $(y_i-y_{i-1}\ge1)$, then they would definitely be placed in separate locations. On the other hand, if the the gap is smaller than one $(y_i-y_{i-1}\leq1)$, they may be mapped to the same location depending on the location boundary.
In addition, the smaller the gap value the more the probability of the keys falling in the same location.

The gap values are constrained by the condition that the sum of all the gaps should be less than $\left(N-1\right)$\footnote{Sum of gaps is: $\sum_{t=1}^{N-1}\left(y_t-y_{t-1}\right) =y_{N-1}-y_{0} \leq N-1$}, and thus, the mean gap value turns out to be less than or equal to one ($E[G] \leq 1$). 
Ideally, we would want all the gaps to be exactly equal to one as this leads to zero collisions and also satisfies the constraint.
Qualitatively speaking, any increase in the variance of gap distribution $G$ leads to an increase in the number of gaps below value one and thus, a subsequent increase in the number of collisions.

% \kapil{Can we move the next para to the appendix?}
% If we assume that $g_i$'s are generated from an independent and identically distributed (iid) variable with probability density function $f_{G}(x)$, then the expected number of empty slots $e$, after mapping keys to their hash outputs, is given by the formula below:
% $$\mathbf{E}[e]=N  \cdot  \int_0^1 (1-x)\cdot f_{G}(x) dx $$
% This equation was derived using the fact that if the gap value $x$ is less than one, then with probability $x$, a location boundary would fall between the two consecutive values.
% This is because the location boundaries are separated by unit values and the probability of a random boundary falling in a gap of size $x$ is $x$.
% The probability that no boundaries fall in a gap of size $x$ is $(1-x)$ and $(1-x)*f_{G}(x) dx$ represents the proportion collisions for gap values from [$x,x+dx$].  
% This quantity is then integrated from $0$ to $1$, as consecutive keys with gaps beyond one don't collide.

\noindent\textbf{Collisions for Linear Models.}
The output distribution for linear models is dependent on the input distribution.
% \kapil{are these two examples helpful? maybe we can skip them.}
% To elaborate, we look at two simple examples.
% For sequential input (Input={0, 10, 20, 30, 40, ...}),  a simple linear model ($f(x) = x/10$) would produce perfect mapping and have zero collisions.
% For inputs generated from uniform distribution, a simple linear model would just scale the values and the output distribution would be uniformly distributed in range $[0,N-1]$.
% Thus, the collisions are dependent on the input distribution and the model.
Linear operations scale and offset the input values to obtain the output.
For sorted input values (${x_0,x_1,x_2,..}$), a simple linear model ($y=m * x+b$) will just scale the gaps of the input ($g_i=y_{i+1}-y_{i}=(x_{i+1}-x_{i})*m$).
For piece-wise linear models, the gap distribution of the output values $G$ is a scaled version of the input. The scaling will be such that the mean of $G$ is less than equal to one ($E[G]\leq 1$). 
If the input gap distribution has higher variance, this would be propagated to $G$, leading to more collisions. 
%If the input gap distribution has higher variance, this would be translated to the output gap distribution leading to more collisions. 

Next, we qualitatively argue why more models do not necessarily reduce the number of collisions.
Suppose the input data was generated using a gap distribution $H$ with corresponding PDF $f_H$.
Piece-wise linear models would simply scale different ranges of the input and thus, the corresponding output gap distribution would just be a scaled version of $f_H$. Increasing the number of models does not alter the gap distribution of the output values and thus, the number of collisions stays the same.
In an extreme case, when the number of models is close to the number of keys, then the collisions would be low but the space overhead would make the structure practically unusable.   
% \tim{This is not entirely true. the more models you have, the more you memorize and start to overfit. In the extreme case you could have one model per two data points. You need to at least explain that part}

Here, we visualize the gap distribution of the output values for various datasets and the corresponding proportion of empty slots.
We used piece-wise linear models for various datasets and obtained the output $y_i's$ (CDF) values for them. 
In Figure~\ref{fig:gap_distribution}, we show the PDF of the gap distribution and the proportion of empty slots for three real datasets from~\cite{sosd_bench} and a synthetic uniform one.
Clearly, the gap distribution is much more predictable for \textit{wiki} than for uniform, \textit{fb} and \textit{osm}. 
\textit{wiki} has a gap distribution concentrated more towards one and so ends up having the least number of empty slots.
\textit{osm} tends to have a lot of gaps concentrated towards zero and ends up with the most empty slots.
We provide a formal analysis for the collisions and its relation with gaps distribution in Appendix~\ref{app:collisions}.


\begin{figure}
    \begin{center}
    \includegraphics[width=6cm,height=4cm]{figures/gap_distributions.png}
    \end{center}
    \caption{Gap distribution and effect on collisions}
    % \caption{Probability density functions of the gaps between consecutive output values for various datasets after using piece-wise linear models for hashing. We also show the corresponding proportion of empty slots.}
    \label{fig:gap_distribution}
\vspace{-2mm}    
\end{figure}


\noindent\textbf{Collisions for Hash Functions.} 
In case of a good hash function (e.g., Murmur), the output values will be  uniformly distributed in the range $[0,N-1]$ irrespective of the input distribution. 
Therefore, the gap distribution of the output values is a fixed distribution which corresponds to the uniform case in Figure~\ref{fig:gap_distribution}.

\noindent\textbf{Summary.}
If the input keys are generated from a distribution, then the CDF of the distribution maps the data uniformly randomly in the range $[0,1]$.
Hence, the CDF will behave as an order-preserving hash function in a hash table.
A learned model that approximates this underlying distribution would only be as effective as a hash function in terms of collisions.
In this case, over-fitting to the data is necessary to reduce the collisions. 
If the data is generated in an incremental time series fashion ($x_0,x_1=x_0+g_0,x_2=x_1+g_1,....$), the predictability of the gaps determines the amount of collisions. 
In certain cases, like the \textit{wiki} distribution, a learned model can lead to fewer collisions.
Auto generated IDs with some deletions are the other common case where learned models can beat hash functions. 

% \tim{Two points you want to make in this section: (1) It is how predictable the dataset is. Wiki is very predictable, Uniform isn't. (2) you should make the connection to overfitting as well and explain the meaning of the underlying distribution vs the observered distribution. }
% \tim{The section is overall not easy to follow. It would help a lot to have an example in the first part with the notation.}
% \tim{I would also add an example section and explicitly point out that: (1) a dataset created from a uniform distribution will work not well. Even though a linear model will perfectly capture the underlying CDF, it will not be a better hash function.. (2) auto-generated IDs with deletes are almost a perfect case. Very predictable and arguably also a non-uncommon case }

% \noindent\textbf{Factors affecting Collisions:} 
% If two inputs are mapped to the same location, then there is a collision.
% The amount of collisions is clearly determined by the distribution of the output values. 
% In case of a hash function, the output values would be uniformly distributed in the range $[0,N-1]$ irrespective of the input distribution. 
% Thus, collisions for hash functions are independent of the input distribution. 
% On the other hand, linear models scale and offset the input values to obtain the output.
% The output distribution for linear models is dependent on the input distribution as well as the model.

% To elaborate, we look at two simple examples.
% For sequential input (Input={0,10,20,30,40,...}),  a simple linear model($f(x)=x/10$) would produce perfect mapping and have zero collisions.
% For inputs generated from uniform distribution, a simple linear model would just scale the values and the output distribution would be uniformly distributed in range $[0,N-1]$.
% Thus, the collisions are dependent by the input distribution and the model.


% \noindent\textbf{Effect of Input Distribution on Collisions:}
% The key insight regarding collisions is that the collisions depend on the gaps between consecutive output values (${g_0=y_1-y_0, g_1=y_2-y_1,g_2...}$).
% If the gap between two consecutive output values is greater than one $(y_i-y_{i-1}\ge1)$, then they would be placed in separate locations whereas if the the gap is smaller than one $(y_i-y_{i-1}\leq1)$, they maybe mapped to the same location depending on the location boundary.

% In the previous example of sequential and uniformly distributed inputs, the gap values for sequential are always constant whereas for uniform distribution they are non-constant but have a certain fixed distribution.
% These non-constant gaps distribution lead to more collisions for uniformly distributed inputs.
% Intuitively, more variance in the gaps also leads to more collisions.

% Here we try to formally argue these claims.
% We model the sorted input($x_0,x_1,.$) as a stream generating the gaps $g_1,g_2,...$ where $x_i=\left(\sum_{t=1}^i g_t\right)+x_0$.
% The gaps $g_1,g_2,...$ form a gap distribution $G$ with pdf $f_g$.
% These input values($x_i$) are mapped to output locations($f(x_i)=y_j$), shown in sorted order as $y_0,y_1,...$ where each $y_i\in [0,N-1]$.
% The output values generate a set of gaps $g^{'}_1, g^{'}_2,...$ such that $y_i=\left(\sum_{t=1}^i g^'_t\right)+y_0$. 
% These gaps forms a gap distribution $G^'$ with pdf $f_{g^'}$. If we have $y_0=0$ and $y_{n-1}=n-1$, the mean \footnote{The mean is ($\left(\sum_{t=1}^{i} g_t\right)/(n-1)$) which is equal to $\left(y_{n-1}-y_0\right)/(n-1)$.} of $G^'$ will be $1$.  
% For a perfectly random hash functions, the gap distribution of the output values is a fixed distribution.
% % To simplify the analysis of learned model, we just consider a simple linear model to be our learned model.
% For sorted input values (${x_0,x_1,x_2,..}$), a simple linear model($y=m\times x+b$) will just scale the gaps of the input ($g_i=(x_{i+1}-x{i})m$).
% So in the case of picewise scaled linear learned models, the gap distribution of the output values simply is a scaled version of the input.


% If we assume that $g_i$'s are generated from an independent and identically distributed (iid) variable with probability density function ($f_{g^'}(x)$), then the expected number of empty slots($e$) after mapping is given by the formula below:

% $$\mathbf{E}[e]=N  \cdot  \int_0^1 (1-x)\cdot f_{g^'}(x) dx $$


% \noindent\textbf{Can more models help reduce collision?}








% \begin{itemize}
%     \item What are collisions dependent on?
%     \item Gap Based Theory (Birthday Variant)
%     \item Evaluation on conflict rate based on gap distribution
% \end{itemize}

==> Learned Hashing/applications.tex <==
\section{Applications}

\begin{itemize}
    \item Usage in Hash Tables
    \item Cuckoo Hashing
\end{itemize}


==> Learned Hashing/background.tex <==
\section{Background}
\label{sec:background}

\input{background_hash_functions_and_tables}
\input{background_learned_models}
\input{background_parallelism_optimizations}




==> Learned Hashing/background_hash_functions_and_tables.tex <==
%\subsection{Hash Functions}
\noindent\textbf{Hash Functions and Tables.} Murmur~\cite{RAD15} and XXH3~\cite{XXHash} are among the most widely-used hash functions, which have good balance between computation time and collision rates. They are implemented with arithmetic (e.g., multiply, add) and logical (e.g., shift, XOR) operations. However, XXH3 is specifically designed for streaming data. AquaHash~\cite{AquaHash} is another popular hash function that leverages Advanced Encryption Standard (AES) instructions~\cite{AES}. In general, hashing schemes for handling collisions are categorized into two main categories: chaining and open addressing. Bucket chaining~\cite{BTA+13} is a standard hash table implementation that follows the chaining scheme. It contains a set of $n$ buckets, where each bucket has a pre-allocated array of $s$ entries. On an insert, once a collision occurs, the item is inserted in the current available entry in its corresponding bucket. If the current bucket is already filled up, a new one is created, pre-allocated and chained to it. For open addressing scheme, Cuckoo hash table~\cite{PR04} has become the recent state-of-the-art.
Every item has two possible locations: its primary and its secondary bucket.
When inserting an item and its primary bucket is full, it gets placed into its secondary bucket.
If the secondary bucket is also full, a random item is kicked from the bucket and is placed into its alternative location (balanced kicking).
In contrast, biased kicking~\cite{cuckoo-index} prefers kicking items that reside in their secondary buckets.
The idea behind this is to increase the ratio of items in their primary buckets (primary ratio) and hence improve performance for positive lookups.
Typically, Cuckoo hashing is implemented with two independent hash functions.
%For details about the performance of chaining and Cuckoo hash tables under different scenarios and workloads, refer to the experimental study in ~\cite{RAD15}.




%Hashing has been extensively investigated for decades.
%Multiply-shift~\cite{DHK+97}, Multiply-add-shift~\cite{Die18}, and Murmur~\cite{RAD15} are among the most widely-used hash functions, which have good balance between computation time and collision rates. They are implemented with arithmetic (e.g., multiply, add) and logical (e.g., shift, XOR) operations. %, and hence can be efficiently vectorized. 
%Perfect hashing~\cite{DKM+94} is another family of functions that produce exactly zero collisions, yet are quite expensive to build and compute. Minimal perfect hashing (e.g., RecSplit~\cite{EGV20}) additionally ensures mapping $n$ keys to exactly $n$ hash buckets (i.e., no extra space cost). 


%\noindent\textbf{Hash Functions.} Hashing has been extensively investigated for decades. Here, we just highlight some of the well-known functions: 1) \textit{Multiply-shift}~\cite{DHK+97} and \textit{Multiply-add-shift}~\cite{Die18} are extremely fast functions with strong theoretical guarantees for collision probabilities. They can be implemented with efficient multiply, add, and shift instructions. %However, Multiply-add-shift requires 128-bit arithmetic operations for hashing 64-bit keys, which rarely have built-in support by current hardware. 2) \textit{Murmur}~\cite{RAD15} is a well-engineered hash function, with no proven theoretical guarantees. It is implemented with a bunch of multiply, shift, and XOR operations, and can be efficiently vectorized. 3) Perfect hashing~\cite{DKM+94}  is a family of functions that produce exactly zero collisions, yet are quite expensive to build and to compute. Minimal perfect hashing (e.g., RecSplit~\cite{EGV20}) additionally ensures mapping $n$ keys to exactly $n$ hash buckets (i.e., no extra space cost).


%\subsection{Hash Tables}
%\noindent\textbf{Hash Tables.} Hashing collision schemes are mainly categorized into two main categories: chaining and open addressing. We give a brief description for a representative hash table implementation in each category. For chaining, bucket chaining~\cite{BTA+13} is a standard table which contains a set of $n$ buckets. Each bucket has a pre-allocated array of $s$ entries. On an insert, once a collision occurs, the item is inserted in the current available entry in its corresponding bucket. A new bucket is created, pre-allocated and chained to the current one if the current one is already filled up. For open addressing, Cuckoo hash table~\cite{PR04} is a state-of-the-art data structure that, in its simplest form, contains two hash tables with two independent hash functions. Every inserted item is stored at either one of these tables, but never in both. When inserting an item, and if its corresponding bucket in the first table is not empty, the existing item in this bucket is kicked out to store the current input item, and the removed item is tried to be inserted in the second table. For details about the performance of chaining and Cuckoo hash tables under different scenarios and workloads, refer to the experimental study in ~\cite{RAD15}.


==> Learned Hashing/background_learned_models.tex <==
%added by Ibrahim
%\subsection{Learned Models}

\noindent\textbf{Learned Models.} Recently, the idea of using learned models to predict the location of keys in datasets has gained a great attention in the database community~\cite{KBC+18}. {\rmi}~\cite{KBC+18} was the first proposed index that uses multi-stage learned models. In {\rmi}, the root model gives an initial prediction of the CDF for a specific key. Then, this prediction is recursively refined by more accurate models in the subsequent stages. Interestingly, the authors of~\cite{KBC+18} also discussed the idea of using CDF-based learned models as order-preserving hash functions, which is the main scope of this paper. An interesting index that followed {\rmi}, namely {\rs}~\cite{KMR+20}, employs a radix table to quickly find the two spline points that approximate the CDF for a specific key. Then, linear interpolation between the retrieved spline points is used to locate the key.  In this paper, we only focus on piece-wise linear models that are built using a set of line segments, where each segment is represented by a slope and an intercept. Both {\rmi} and {\rs} can be considered as piece-wise linear models, which are just trained/created in a different way. 
%In this paper, we focus on using piece-wise linear models as used by {\rmi}, {\rs}, and {\pgm}.

%In this paper, we investigate the usage of {\rmi}, {\rs}, and {\pgm} as hash functions.

%In {\pgm}, the learned models follow a multi-level structure as in {\rmi}, yet, each level represents an error-bounded piece-wise linear regression. 

%In general, all learned models require training parameters (e.g., intercepts and slopes for linear models) that will be used to estimate the CDF values of testing keys. 


==> Learned Hashing/background_parallelism_optimizations.tex <==
%added by Ibrahim
% \noindent\textbf{{\simd} and Prefetching-optimized Execution.} Single Instruction Multiple Data ({\simd}) instructions allow operating a single instruction on a vector of data in parallel, and hence increase the data level parallelism. Recently, the length of the vector registers supported by {\simd} became 512 bits in the latest {\avx} instruction set. {\simd} has been heavily studied in different database operations (e.g.,  scanning~\cite{LMF+16, DKF+18}, joins~\cite{FZW19, FHC+19}, sorting~\cite{CNL+08, IT15}), and systems that employ the vector-at-a-time execution model~\cite{ZR02, PRR15, KLK+18}. Meanwhile, prefetching-optimized inter-task parallelism techniques were proposed to hinder cache misses, including Group Prefetching ({\gp})~\cite{CAG+07}, Asynchronous Memory Access Chaining ({\amac})~\cite{KFG15}, and Coroutines~\cite{PLM+17, JMH+18}. In these techniques, when a task issues a memory prefetching, the execution switches to other tasks in the pipeline to keep busy, and then returns to process the prefetched data after a while. In this paper, we use {\amac} due to its simplicity.
% \tim{This section seems not really related work, more like implementation details. If you need space, this part can be removed. Instead you might want to explain RMI}

%\noindent\textbf{Single Instruction Multiple Data ({\simd}).} Modern processors are equipped with {\simd} instructions that allow operating a single instruction on multiple data elements (i.e., vector of data) in parallel, and hence increase the data level parallelism. The length of the vector registers supported by {\simd} increased over time and, recently, became 512 bits in the latest {\avx} instruction set. This allows the processing of an entire cache line with a single instruction only. {\simd} has been heavily studied in different database operations (e.g.,  scanning~\cite{LMF+16, DKF+18}, joins~\cite{FZW19, FHC+19}, sorting~\cite{CNL+08, IT15}), and systems that employ the vector-at-a-time execution model~\cite{ZR02, PRR15, KLK+18}.

%{\simd} has been heavily studied in the data management field to accelerate different operations, including scanning~\cite{LMF+16, DKF+18}, bloom filters~\cite{PR14}, joins~\cite{FZW19, FHC+19}, sorting~\cite{CNL+08, IT15}, and set intersection~\cite{IOT14}, as well as interpret database systems that employ the vector-at-a-time execution model~\cite{ZR02, PRR15, KLK+18}. 
%In general, the {\simd} vectorized execution helps such database operations and systems to reduce both computation overhead and branch misses.

%full vectorization~\cite{PRR15} 

%\noindent\textbf{Prefetching-optimized Execution.} Cache misses become a major bottleneck in in-memory operations (e.g., join~\cite{CAG+07}, indexing~\cite{JMH+18}). The overhead of such cache misses can be effectively hindered by loading data beforehand into cache through \textit{software prefetching}. However, prefetching is incapable of improving the caching performance if the time between knowing the data addresses and processing such data is much less than the desirable prefetching distance (i.e., immediate memory access).
%(e.g., when traversing an index, the addresses of next nodes are not known until current nodes are processed). 
%In such case, an \textit{immediate memory access} is required.
%To handle this situation, prefetching-optimized inter-task parallelism techniques were proposed including Group Prefetching ({\gp})~\cite{CAG+07}, Asynchronous Memory Access Chaining ({\amac})~\cite{KFG15}, and Coroutines~\cite{PLM+17, JMH+18}. In these techniques, when a task issues a memory prefetching, the execution switches to other tasks in the pipeline to keep busy, and then returns to process the prefetched data after a while.

%Cache misses become a major bottleneck in in-memory database operations, such as join~\cite{CAG+07}, sorting~\cite{IT15} and indexing~\cite{JMH+18}.

%{\simd} counter control divergence~\cite{LPK+20}, Combining SIMD and prefetching: (ROF)~\cite{MMP17}, IMV~\cite{FZW19}



==> Learned Hashing/conclusion.tex <==
\vspace{-5pt}
\section{Conclusion}

Learned models can indeed provide better collision profile than hash functions in certain situations depending on the gap distribution of the input.
With learned models it is hard to beat hash functions in computation time, without the support of vectorization and prefetching-optimized execution techniques.
Bucket chaining hash tables can greatly benefit from learned models to save extra space overhead along with some minor benefits in probe times.
Similarly, Cuckoo hash tables can improve their primary key ratio using learned models and achieve a slightly better probe latency.


==> Learned Hashing/evaluation.tex <==
\section{Evaluation}
% \kapil{We should have 2d scatter plots for the graphsChained: probe latency and space usedCuckoo: probe latency and primary key ratio}
\label{sec:evaluation}

% In the evaluation, we want to back up the following claims:
% \begin{itemize}
%     \item Learned Models can be as fast as hash functions
%     \item Learned Models can lead to lower collisions in certain cases
%     \item Learned models can improve the probe time and space used by chained hash tables
%     \item Learned Models improves the primary bucket ratio and probe time for cuckoo hash tables.
% \end{itemize}

For the experiments, we use three real datasets from \cite{sosd_bench}, namely \textit{wiki}, \textit{osm}, and \textit{fb}, in addition to three variations of a synthetic sequential dataset with different x\% elements removed randomly (x=\{0, 1, 10\}). 
Each real or synthetic dataset has around 200 million 64-bit keys. We de-duplicate the real datasets before using them.
We use AquaHash~\cite{AquaHash}, XXH3~\cite{XXHash} and Murmur~\cite{Murmur3} with fast modulo reduction\footnote{Modulo reduction is based on efficient integer division (https://libdivide.com).} as traditional hash functions and two efficient learned models: {\rmi}~\cite{KBC+18} and {\rs}~\cite{KMR+20}. 

\noindent\textbf{Computation Time.} Figure~\ref{fig:computation_time} shows the median throughput for hashing the sequential dataset with 10\% removed elements using traditional hash functions and non-vectorized learned models, while varying the count of line segments used in each model. As expected, traditional functions are much better than non-vectorized learned models, even with small sizes. The throughput of learned models decreases significantly for large sizes due to the increased number of cache misses when accessing the model parameters. Table~\ref{table:rmi_compute} shows the performance of {\amac}-based vectorized versions of both {\rmi} and Murmur hashing for the same dataset. As shown, with $10^3$ models, the performance gap between non-vectorized {\rmi} and Murmur is substantial (around 10 ns difference), however, using the {\amac}-based vectorization reduces this gap to be 2 ns only. Note that, at very large models (e.g., $10^7$), {\rmi} becomes much slower than Murmur, even with vectorization.




%Here, we look at the average computation for hash functions and learned models.
%The computation time for {\rmi}'s is dependent on the architecture of the model, so we vary the number of model for this experiment.
%The computation time for the techniques are shown in Figure~\ref{fig:computation_time}. The computation time for {\rmi}'s increases significantly with the architecture due to the increasing cache misses. Hash functions are much better than even {\rmi}'s with small architecture.

%In Table.\ref{table:rmi_compute}, we show the RMI computation time for vectorized and non-vectorized versions with increasing model sizes.
%A model with $10^7$ models in second level would incur a L2 cache miss which can be avoided by vectorizing and hence the computation time difference is significant. 
%, and provides a competitive running time with state-of-the-art traditional hash functions.


%\begin{figure}
%    \begin{center}
%    \includegraphics[]{figures/median_throughput.pdf}
%    \end{center}
%    \caption{Median throughput (10 runs) (\textbf{not} latency, i.e, full interleaving etc possible). For {\rs} only the fastest numbers are shown where different configurations produced the exact same model count (heavy deviation in speed due to \textit{radix bits} parameter). For Murmur, the median value over various datasets was taken (seemed fair, variation was minor anyways).}
%    \label{fig:computation_time}
%\end{figure}

%\begin{figure}
%     \centering
%     \begin{subfigure}{0.5\textwidth}
%         \centering
%         \includegraphics[]{figures/median_throughput.pdf}
%         \caption{Median throughput}
%         \label{fig:computation_time}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.5\textwidth}
%         \centering
%         \includegraphics[]{figures/empty_slots.pdf}
%         \caption{Empty slots (percentage)}
%         \label{fig:collisions}
%     \end{subfigure}
%     \caption{Effect on Computation time and Collisions.}
%     \label{fig:computation_time_and_collisions}
%\end{figure}

\begin{figure}
     \centering
     \subfigure[Median keys per  second]{\includegraphics[width=1.6in,height=2.7cm]{figures/median_throughput.pdf}
     \label{fig:computation_time}}
     \subfigure[Empty slots (percentage)]{\includegraphics[width=1.6in]{figures/empty_slots.pdf}
     \label{fig:collisions}}
     \caption{Throughput and collisions comparisons.}
     \label{fig:computation_time_and_collisions}
\end{figure}



\begin{table}
\small
\begin{tabular}{|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}\scriptsize{Model} \\ \scriptsize{Count} \end{tabular} & \begin{tabular}[c]{@{}l@{}}\scriptsize{Non-Vect.} \\ \scriptsize{Murmur (ns)} \end{tabular} & \begin{tabular}[c]{@{}l@{}}\scriptsize{Vect.} \\ \scriptsize{Murmur (ns)} \end{tabular} & \begin{tabular}[c]{@{}l@{}}\scriptsize{Non-Vect.} \\  \scriptsize{RMI (ns)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\scriptsize{Vect.}  \\  \scriptsize{RMI (ns)}\end{tabular} \\ \hline
10       & 2.4 & 1.9 & 10 & 4 \\ \hline
$10^3$   & 2.4 & 1.9 & 13 & 4 \\ \hline
$10^5$   & 2.4 & 1.9 & 25 & 8 \\ \hline
$10^7$   & 2.4 & 1.9 & 112 & 22 \\ \hline
\end{tabular}
\caption{Computation time of vectorized {\rmi} and Murmur.}
\label{table:rmi_compute}
\vspace{-10mm}
\end{table}

\noindent\textbf{Collisions.} Figure~\ref{fig:collisions} shows the amount of collisions for {\rs} against Murmur hashing on various datasets. {\rmi} is omitted as it has similar results to {\rs}. Here, we mapped $N$ elements into $N$ slots and report the proportion of empty slots. The dashed line is the theoretically expected value for true uniform random hash functions. As shown in the figure, for many datasets, learned models indeed have less empty slots than hash functions (i.e., less collisions). However, for \textit{fb} and \textit{osm} datasets, the models make the collisions worse. This confirms our analysis in Section~\ref{sec:analysis_collisions}.

%Here, we analyze the amount of collisions for hash functions and learned models on various datasets. We mapped $N$ elements into $N$ slots and report the proportion of empty slots in Figure~\ref{fig:collisions}. In this figure, Dashes line is the theoretically expected value for true uniform random hash functions.
%We used a {\rs} model with -- error and -- config. For some real world datasets, learned models indeed have less empty slots than hash functions. For other distributions, the models make the collisions worse. This has to do with the gap distribution as discussed in Sec.\ref{sec:analysis_collisions}.

%\begin{figure}
%    \begin{center}
%    \includegraphics[]{figures/empty_slots.pdf}
%    \end{center}
%    \caption{Empty slots (percentage)over various datasets at load factor == 1. Dashes line is the theoretically expected value for true uniform random hash functions.}
%    \label{fig:collisions}
%\end{figure}


\begin{figure}
    \begin{center}
    \includegraphics[width=3in]{figures/hash_combined.pdf}
    \end{center}
    \caption{(a)~Bucket chaining hash table probe times for varying payload sizes and slots per bucket. (b)~Primary key ratio and probe times for various kicking strategies and load factors.}
    \label{fig:primary_key}
\end{figure}

% \begin{figure}
%     \begin{center}
%     \includegraphics[width=3in]{figures/cuckoo.pdf}
%     \end{center}
%     \caption{Primary key ratio (percentage) and corresponding probe times over various datasets.}
%     \label{fig:primary_key}
% \end{figure}

\noindent\textbf{Bucket Chaining Hash Tables.} Bucket chaining hash tables deal with collisions by creating linked lists for the keys mapped to the same location. When retrieving a key, we traverse the linked list until we find the key. With increased collisions, the space needed for the chained hash tables increases. Figure~\ref{fig:primary_key}(a) shows the effect of using different hash functions and {\rs} as a representative learned model when building bucket chaining hash tables with different payload and bucket sizes. We observe that {\rs} can lead to less probe times for all of the datasets, except \textit{fb} and \textit{osm} ones. Moreover, larger payloads lead to larger cache miss penalties, and hence with increasing payload sizes, hash functions take slightly more time than learned models.

%We observe that, with increasing slots per bucket, the effect of collisions decreases, and hence the difference between additional buckets used by hash functions is less evident. Moreover, larger payloads lead to larger cache miss penalties, and hence with increasing payload sizes, hash functions take slightly more time than learned models.

\noindent\textbf{Cuckoo Hash Tables.} %Cuckoo hash tables reduce the number of collisions by having multiple potential locations for a key. The primary key ratio refers to the amount of keys that are in their first potential location. 
Having a high primary key ratio reduces the amount of unnecessary lookups, as one avoids going to the second location, and hence improves the probe time. We show the effect of replacing one of the used multiple hash functions by a learned model. We use a Cuckoo Hash with 2 hash functions, load factor of 1, bucket size of 8, and two kicking strategies; balanced and biased~\cite{cuckoo-index}. As shown in Figure~\ref{fig:primary_key}(b), using any two traditional hash functions consistently achieves primary key ratios of 62\% and 83\%, for biased and balanced kicking, respectively, which are close to theoretically optimal. However, we observe that using learned models, e.g., {\rs}, along with both kicking strategies can lead to better primary key ratio for all of the datasets, except \textit{fb} and \textit{osm} ones.
% Balanced kicking nullifies the advantage of using a hash function which provides better primary key ratio unlike biased kicking.
% Random 
With biased kicking, learned models get a much better primary key ratio which leads to lower cache misses and thus a slightly better probe time.
% \tim{I really don't know how to read Figure 3. The primary key ratio has no real meaning for the performance, does it? Lower means better? Why is that experiment not done with different payloads? This seems to be much more important }
%Cuckoo hash tables reduce the number of collisions by having multiple potential locations for a key using multiple hash functions. When retrieving a key, we check multiple locations in order until we find the key. The primary key ratio refers to the amount of keys that are present in their first location. 
%Having a high primary ratio ensures that the amount of unnecessary lookups is reduced. 
%Here, we show that replacing one of the hash functions by learned model one can achieve a better primary key ratio. We use a Cuckoo Hash with bucket size 4 and 2 hash functions for this experiment along with biased kicking. The results for this experiment are shown in Figure~\ref{fig:primary_key}. The cuckoo hash table with both hash functions consistently achieves a primary ratio of 83\% which is close to theoretically optimal. The primary ratio for learned model based Cuckoo table varies based on data and is worse for FB and OSM datasets.
%The probe time of learned model based table however is similar or worse than hash functions based table.
%We observe the following trends w.r.t kicking strategy and load factor on datasets favourable for learned hash.
%Biased Kicking leads to better primary key ratio for both learned models and hash functions. 
%Higher lead factor slightly decreases the primary key ratio.



\begin{figure}
     \centering
     \subfigure[16 bytes payloads]{\includegraphics[width=1.6in,height=2.7cm]{figures/probe_times_overall_16.pdf}}
     \subfigure[64 bytes payload]{\includegraphics[width=1.6in,height=2.7cm]{figures/probe_times_overall_64.pdf}}
     \caption{Probe times comparison between Cuckoo and bucket chaining hashing.}
     \label{fig:probe_times_comparison}
\end{figure}
%We used learned models and Murmur hashing as the hash functions in chained hash tables.
%Figure~\ref{fig:chained_stuff} shows the space used v/s probe time by chained hash tables for 2 different payload sizes and slot sizes. For some datasets, learned hash indeed has both better probe time and space used than Murmur hashing. 
%We observe the following trends w.r.t payload and slots on datasets favourable for learned hash.
%With increasing slots per bucket, the effect of collisions decreases and hence, the difference between additional buckets used by hash functions is less evident. 
%Larger payloads lead to larger penalties for cache miss and hence with increasing payload sizes hash functions take slightly more time than learned models.
% \begin{figure}
%     \begin{center}
%     \includegraphics[width=3in]{figures/chained.pdf}
%     \end{center}
%     \caption{Bucket chaining hash table probe times for various payload sizes and slots per bucket. }
%     \label{fig:chained_stuff}
% \end{figure}



\noindent\textbf{Combined Probe Times.}  Figure~\ref{fig:probe_times_comparison} shows the probe times achieved by employing each of {\rs} and Murmur hashing inside both bucket chaining and Cuckoo hash tables on various datasets. We used bucket size of 4 for both tables. Also, biased kicking is used for constructing the Cuckoo table. As shown, for all datasets except \textit{fb} and \textit{osm}, bucket chaining with {\rs} is the best strategy. Cuckoo tables are generally slower than their chained counterparts.

%In Figure~\ref{fig:probe_times_comparison}, we compare the probe times achieved by hash functions and learned models along with chaining and cuckoo hashing strategies on various datasets.  We use bucket size 4 for chained and cuckoo tables, biased kicking is used for constructing cuckoo tables.
%In the figure, for all datasets except \textit{fb} and \textit{osm}, learned models with chaining is the best strategy. Cuckoo tables are generally slower than their Chained counterparts. 




% \newpage
% \textbf{DataSets}


% \begin{itemize}
%     \item Synthetic: Vary gap distribution of uniform random distribution to generate various synthetic datasets. 
%     \item Real: WebLogs, Genome, Longitude, FB, Wiki, etc
% \end{itemize}

% \textbf{Hash Functions}
% For multiplicative methods, the more significant bits are of higher quality due to the nature of the multiplication operation. Therefore, shifting is commonly used before applying other reduction techniques to ensure that the least-quality, i.e., the bottom bits, are discarded first.

% \textbf{Reduction Methods}
% Magic constants (state of the art), Lemire's fastrange, modulo. For multiplicative methods, it could be beneficial to rightshift first before applying other reduction techniques.

% \textbf{Hash Tables}
% Robinhood Hash, Chained Hashing, Linear Probing, Quadratic Probing, Cuckoo Hashing, 

% \subsection{Learned Hash function Evaluation}

% \subsubsection{Main Expt 1: RMI Latency vs Hash Function Latency no-batch/batch Processing}

% Claim: RMI's can be as fast as a hash function even when no batch processing.

% Claim: For batch processing similar latencies



% \subsubsection{Main Expt 2: RMI collision Rate vs Hash Functions on various datasets}
% Show num elments in a bucket.
% Claim: RMI Collisions depend on gap distribution and depending on the data it can be better than Hash Function

% \subsubsection{Micro Expt 1: RMI accuracy/memory usage vs collision rate}

% Claim: Accuracy of the model and Collision Rate are orthogonal 


% \subsubsection{Micro Expt 2: RMI latency as we increase its size}

% Claim: Latency stays more or less similar



% \subsection{Learned Hash Function in Hash Maps}

% \subsubsection{Main Expt 1: Lookup Time for various Hash Maps with/without using RMI as Hash function on various datasets for various Load Factors}
% While measuring lookup time vary unsuccessful lookup ratio.
% Generate a huge table with color shades indicating the relative performance.
% Claim: On the datasets for which we have lower RMI collisions, Lookup time improves


% \subsubsection{Micro Expt 1: Insertion Time for various Hash Maps with/without using RMI as Hash function on various datasets For various Load Factors}

% Claim: On the datasets for which we have lower RMI collisions, Insertion time improves

% \subsubsection{Micro Expt 2: Construction Time of the RMI}

% Claim: RMI is pretty fast to construct and does not add significant overhead to the Hash Map construction time.

% \subsection{Learned Hash Function in Joins}

% \textbf{Hash Join}
% Not useful as if uncorrelated predicate is applied the data is almost random.

% \textbf{Hash Index Nested Loop Join}
% \subsubsection{Main Expt 1: Join Time for Chained Hash Map with/without using RMI as Hash function on various datasets}

% Claim: Join faster on sequential and other predictable datasets.



==> Learned Hashing/introduction.tex <==
\section{Introduction}

Hashing is a fundamental operation in computer science and commonly used in databases~\cite{RAD15}. They are mainly used to accelerate point queries, perform joins and grouping, etc. (e.g.,~\cite{BTA+13, JMH+18}).
 In hash tables, a key is mapped to a location in constant time (i.e., $O(1)$).
Compared to the traditional tree-structured main-memory indexes, hash tables have been proven to be much faster for point queries.
Meanwhile, a lot of data structures and algorithms are recently being enhanced by learned models (e.g.,~\cite{KBC+18, KVC+20}). These learned structures can outperform their traditional counterparts on practical workloads. Along this line of work, the authors of~\cite{KBC+18} introduced the idea of using learned models instead of hash functions, and supported that by some empirical evidence. 
In this paper, we aim to study in more detail when learned models are better hash functions, particular for applications like hash-maps. We primarily consider piece-wise linear models in our analysis as they have small inference times and are sufficiently general to capture complex distributions.

Our study investigates the performance of learned models in terms of: \textit{the number of collisions}, and \textit{the computation time}. 
% \is{The following statement is out of context.} \textcolor{red}{The memory used by the learned models is order of magnitude larger than hash functions but it is much smaller than the memory used by the hash table.}
%We analyze the learned models in terms of: the model computation time and the amount of collisions. 
A collision between two keys occurs when they have the same hash value. Some hash functions are extremely fast to compute, yet, they might suffer from a considerable collision rate in some scenarios (e.g., Multiply-shift~\cite{DHK+97}).
%Some hash functions are extremely fast to compute but a well known issue with hash functions is collisions.
In general, there are known theoretical lower bounds on the number of collisions achieved by hash functions.
We observed that learned models might be able to do better than these lower bounds and outperform hash functions. In particular, it turns out that the amount of collisions for learned models is dependent on the data distribution.
% Our key insight is that, for piece-wise linear models, the predictability of the gaps between consecutive keys in sorted list of keys dictate the number of collisions. \tim{simplify/expand the sentence? Pretty hard to parse. }
% Thus, we conclude that, depending on the data distribution, the amount of collisions can be much better or worse than a hash function.
%learned Models might be able to do better than these lower bounds and outperform hash functions in terms of collisions.
%Note, we primarily consider piece-wise linear models in this work.

Regarding computation time, we empirically found that learned models are slower to compute than most hash functions due to the cache miss overhead from randomly accessing the model's parameters. However, with the help of vectorization and prefetching-optimized inter-task parallelism (e.g., {\amac}~\cite{KFG15}), the learned models computation time can come quite close to its hashing counterpart (around 2 ns difference using models with moderate size).

%We empirically found that most hash functions are faster to compute than learned models but learned models are not far off.
%Vectorized learned model computation can come quite close to the hash function computation times.

% \kapil{motivate why chained and Cuckoo}
To show the effect of using learned models within hashing applications, we built bucket chaining and Cuckoo hash tables using two efficient models, namely {\rmi}~\cite{KBC+18} and {\rs}~\cite{KMR+20}, instead of hash functions.
%As applications we use chained hash tables and Cuckoo Hash tables with learned models instead of hash functions.
Typically, in Cuckoo hashing, a single hash function is used to extract two hash sequences. In our experiments, we computed one hash sequence using the learned model and the other using the hash function.  
% \ak{Why only one hash function? Typically you use a single hash function and then extract the two hash sequences.}
We empirically evaluate the performance of these altered hash tables with various real-world and synthetic datasets.
%For some datasets, learned models indeed perform worse than hash functions. 
For bucket chaining, we found that learned models can achieve 30\% smaller hash tables and 10\% lower probe latency. 
For Cuckoo hashing, in some datasets, learned models can increase the ratio of keys stored in their primary locations (primary key ratio) by around 10\% and a small lookup time benefit in the probe phase.

% \is{Not sure, if we should remove the following contributions or not.}
% \kapil{depends on the space}
% Our contributions include:
% \begin{itemize}
%     \item A comparison of hash functions and learned models w.r.t. computation time and collision rate on various synthetic and real-world datasets.
%     \item An evaluation of hash functions and learned models when used in chaining-based and Cuckoo hash tables.
% \end{itemize}

% Hash Tables are one of the most fundamental data structures.
% A function maps a key to a position in O(1) time.

% \begin{itemize}
%     \item Problems are conflicts, different keys map to the same position
%     \item Cuckoo hashing and bucketization power of two can help with collisions. 
%     \item However, models can outperform hash functions in the number of collisions in certain scenarios
%     \item Models can be faster than hash functions because of weird hardware effects


% \end{itemize}


==> applications.tex <==
\section{Applications}

\begin{itemize}
    \item Usage in Hash Tables
    \item Cuckoo Hashing
\end{itemize}


==> conclusion.tex <==
\vspace{-5pt}
\section{Conclusion}

Learned models can indeed provide better collision profile than hash functions in certain situations depending on the gap distribution of the input.
With learned models it is hard to beat hash functions in computation time, without the support of vectorization and prefetching-optimized execution techniques.
Bucket chaining hash tables can greatly benefit from learned models to save extra space overhead along with some minor benefits in probe times.
Similarly, Cuckoo hash tables can improve their primary key ratio using learned models and achieve a slightly better probe latency.

